Neutron-proton scattering and singular potentials

We consider a Bargmann-type rational parametrization of the nucleon scattering phase shifts. Applying Marchenko's method of quantum inverse scattering we show that the scattering data suggest a singular repulsive core of the potential of the form $2/r^2$ and $6/r^2$ in natural units, for the ${}^3S_1$ and ${}^1S_0$ channels respectively. The simplest solution in the ${}^3S_1$ channel contains three parameters only but reproduces all features of the potential and bound state wave function within one percent error. We also consider the ${}^3S_1$-${}^3D_1$ coupled channel problem with the coupled channel Marchenko inversion method.

==> algebra.tex <==
In this appendix we carry out the last two steps of quantum inverse scattering
for a special class of $F(r)$ functions of the form
\beq
F(r)=-\sum_{m=1}^N\,R_m\,{\rm e}^{-\omega_m r}.
\label{expF}
\eeq
The solution turns out to be completely algebraic \cite{EZB}.

Using this $F(r)$ in the Marchenko equation (\ref{Marchenko}) we obtain
\beq
A(r,u)=\sum_{m=1}^NR_m{\rm e}^{-\omega_m u}\left\{{\rm e}^{-\omega_m r}+\int_r^\infty{\rm d}
t A(r,t){\rm e}^{-\omega_m t}\right\}.
\eeq
We see that the $u$ dependence of $A(r,u)$ must be of the form
\beq
A(r,u)=\sum_{m=1}^N R_m \alpha_m(r){\rm e}^{-\omega_mu},
\label{Ansatz}
\eeq
where
\beq
\alpha_m(r)={\rm e}^{-\omega_m r}+\int_r^\infty{\rm d}t A(r,t){\rm e}^{-\omega_m t}.
\eeq
Using here the Ansatz (\ref{Ansatz}) again we get
\beq
\alpha_m(r)={\rm e}^{-\omega_mr}+\sum_{n=1}^NR_n\,\alpha_n(r)\frac{1}{\omega_m+\omega_n}{\rm e}^{-(\omega_m+\omega_n)r},
\eeq
which can be further simplified by introducing
\beq
\alpha_m(r)={\rm e}^{-\omega_mr}\,\beta_m(r),\qquad\qquad z_m(r)=R_m\,{\rm e}^{-2\omega_mr}.
\eeq
This way we obtain the algebraic equations
\beq
\beta_m(r)=1+\sum_{n=1}^N\frac{z_n(r)\,\beta_n(r)}{\omega_m+\omega_n}.
\label{algebra}
\eeq
The matrix corresponding to this linear problem is
\beq
{\cal M}_{mn}(r)=\delta_{mn}-\frac{z_n(r)}{\omega_m+\omega_n}.
\eeq
${\cal M}$ can be written as
\beq
{\cal M}={\cal K}\Delta,
\eeq
where
\beq
{\cal K}_{mn}=\frac{1}{z_m}\delta_{mn}-\frac{1}{\omega_m+\omega_n},\qquad
\Delta_{mn}=z_m\delta_{mn}.
\eeq
The solution will be expressed in terms of the quantities
\beq
\gamma_m=\sum_{k=1}^N\left({\cal K}^{-1}\right)_{mk},\qquad\quad
{\cal D}={\rm det}({\cal K}).
\eeq
We find
\beq
\beta_m(r)=\frac{1}{z_m(r)}\gamma_m(r),
\eeq
\beq
A(r,u)=\sum_{m=1}^N\gamma_m(r){\rm e}^{\omega_m(r-u)}.
\eeq
Finally, as shown in \cite{EZB},
\beq
q(r)=-2\frac{{\rm d}}{{\rm d}r}A(r,r)=
-2\frac{{\rm d}^2}{{\rm d}r^2}\ln\vert{\cal D}(r)\vert.
\label{Axx}
\eeq

The bound state wave functions can also be calculated algebraically:
\beq
%\begin{split}
f_j(r)=\varepsilon_j(r)+\int_r^\infty{\rm d}uA(r,u)\varepsilon_j(u)=
{\rm e}^{-\kappa_j r}\left\{1+\sum_{m=1}^N\frac{\gamma_m(r)}{\kappa_j+\omega_m}\right\}.
\label{wf}
%\end{split}
\eeq


\subsection{Bargmann-type rational S-matrix}
\label{B1}

Let us consider rational S-matrices of the form
\beq
S(k)=\pm \prod_{j=1}^{\cal N}\sigma_{a_j}(k),
\label{rat}
\eeq
where
\beq
\sigma_a(k)=\frac{a-ik}{a+ik}.
\eeq
For this type of rational S-matrices
\beq
S(0)=\pm,\qquad\qquad S(\infty)=S(-\infty)=\pm(-1)^{\cal N}.
\eeq
The symmetry properties (\ref{syms}) require that the parameters $a_j$ are
either real or come in complex conjugate pairs. Levinson's theorem (\ref{Levi})
can be written in this case in the form
\beq
{\cal N}_+={\cal N}_-+2J+\Delta+p-1,
\eeq
where ${\cal N}_\pm$ is the number of factors with $a_j$ having $\pm$ real part.

For the S-matrix (\ref{rat}) it is easy to calculate the scattering part of the
$F(r)$ function using (\ref{Fs2}). Closing the $k$ integration contour in the
upper half-plane and using the residue theorem we obtain
\beq
F_s(r)=\mp\sum_{{\rm Re}\,a_j>0}2a_j\prod_{k\not=j}\frac{a_k+a_j}{a_k-a_j}\,
{\rm e}^{-a_j r}.
\eeq
This must be supplemented by the bound state part
\beq
F_b(r)=\sum_{j=1}^Js_j{\rm e}^{-\kappa_j r}.
\eeq
Adding the two contributions $F(r)=F_s(r)+F_b(r)$ is of the form (\ref{expF}).
For ${\rm Re}\,a_j>0$,
\beq
\omega_m=a_j,\qquad\qquad
R_m=\pm 2a_j\prod_{k\not=j}\frac{a_k+a_j}{a_k-a_j}=
i{\rm Res}[S(k)]\vert_{k=ia_j}
\eeq
and for the bound state part
\beq
\omega_m=\kappa_j,\qquad\qquad R_m=-s_j.
\eeq
It can happen that $N<{\cal N}_++J$ since some of the $\kappa_j$ and
$a_j$ may coincide. If some $a_j=b=\kappa_j$, the corresponding term
in $F(r)$ is
\beq
(s_j-\hat s_j){\rm e}^{-br}.
\eeq
In the case discussed above, when the S-matrix is associated to a relativistic
quantum field system, $s_j=\hat s_j$ and this exponential is absent from
$F(r)$!

\subsection{Examples}
\label{B2}

We will use the $({\cal N}_+,{\cal N}_-)[J]^\mu$ notation and first consider
the $(3,0)[1]^+$ case. In this case
\beq
S(k)=\sigma_a(k)\sigma_b(k)\sigma_c(k),\qquad a,b,c >0.
\eeq
We define the constants
\beq
\tilde R_a=2a\frac{(b+a)(c+a)}{(b-a)(c-a)},\qquad
\tilde R_b=2b\frac{(a+b)(c+b)}{(a-b)(c-b)},\qquad
\tilde R_c=2c\frac{(a+c)(b+c)}{(a-c)(b-c)}.
\eeq
We will assume that the single bound state coincides with one of the parameters,
$\kappa_o=b$. The corresponding norming constant can be parametrized as
$s_o=y\tilde R_b$ and we write
\beq
F(r)=(y-1)\tilde R_b{\rm e}^{-br}-\tilde R_a{\rm e}^{-ar}-\tilde R_c{\rm e}^{-cr}.
\eeq
We will study two cases: $y=1$ and $y=2$. These are only possible if $b$ is
the smallest (or largest) parameter of the S-matrix since the norming
constant must be positive. The first choice corresponds to the relativistic
quantum field theory motivated case, while the second one can be called
the sign-flip choice.

In the first case where $y=1$ and $N=2$  we have
\beq
\omega_1=a, \quad \omega_2=c, \qquad\qquad 
R_1=\tilde R_a,\quad R_2=\tilde R_c.
\eeq 
 Therefore, this is a  $2\times2$ matrix problem with
\beq
{\cal K}_1=
\begin{pmatrix}
 \frac{{\rm e}^{2ar}}{\tilde R_a}-\frac{1}{2a} &-\frac{1}{a+c}  \\
-\frac{1}{a+c} & \frac{{\rm e}^{2cr}}{\tilde R_c}-\frac{1}{2c}
\end{pmatrix}
\eeq
and can easily be solved
explicitly for general $a$, $b$, $c$. The solution is given in
sect.~\ref{simplest1}.

In the sign-flip case $N=3$ and
\beq
\omega_1=b,\quad \omega_2=a,\quad \omega_3=c,\qquad\qquad R_1=-\tilde R_b,\quad
R_2=\tilde R_a,\quad R_3=\tilde R_c.
\eeq
Furthermore we take $b=1$, $a=2$ and $c=4$. The corresponding $3\times 3$
matrix is
\beq
{\cal K}_2=
\begin{pmatrix}
-\frac{1}{10}{\rm e}^{2r}-\frac{1}{2}&-\frac{1}{3}&-\frac{1}{5}\\
-\frac{1}{3}&-\frac{1}{36}{\rm e}^{4r}-\frac{1}{4}&-\frac{1}{6}\\
-\frac{1}{5}&-\frac{1}{6}&\frac{1}{40}{\rm e}^{8r}-\frac{1}{8}
\end{pmatrix}.
\eeq
From (\ref{Axx}) and (\ref{wf}) we get
\beq
q(r)=\frac{2}{\sinh^2 r}-\frac{12}{\cosh^2 r}
\eeq
and
\beq
f_o(r)=\frac{1}{2}\frac{\sinh^2 r}{\cosh^3 r}=\frac{1}{2}\varphi_o(r).
\eeq
These are the generalized P\"oschl-Teller (PT) potential and its ground state
wave function \cite{PT}.


\subsection{More examples}
\label{B3}

Let us consider more examples. Firstly, we investigate the $(4,0)[1]^+$ case where the scattering matrix is represented as
\beq
S(k)=\sigma_a(k)\sigma_b(k)\sigma_c(k)\sigma_d(k).
\eeq
Without going any further, we observe that $S(k)$ falls into the class of PT type potentials with the degree of singularity $p=3$ according to Levinson's theorem.

As before, we identify the bound state momentum $\kappa_o$ with $b$. We find 
\beq
F(r)=(y-1)\tilde R_b{\rm e}^{-br}-\tilde R_a{\rm e}^{-ar}-\tilde R_c{\rm e}^{-cr}-\tilde R_d{\rm e}^{-dr},
\eeq  
where the $\tilde R_m$-s read
\begin{eqnarray}
\tilde R_a&=&-2a\frac{(a+b)(a+c)(a+d)}{(a-b)(a-c)(a-d)},\quad \tilde R_b=-2b\frac{(b+a)(b+c)(b+d)}{(b-a)(b-c)(b-d)},\\ 
\tilde R_c&=&-2c\frac{(c+a)(c+b)(c+d)}{(c-a)(c-b)(c-d)},\quad \tilde R_d=-2d\frac{(d+a)(d+b)(d+c)}{(d-a)(d-b)(d-c)}.
\end{eqnarray}

We now use the complex parameters of \cite{BP} (although the symbolic solution is easily obtained by Mathematica):
\beq
a=1.2293,\quad b=0.2315,\quad c=2.5603+3.5248i,\quad d=c^*.
\eeq 
We note that this choice of the parameters yields, once more, a real and positive $\tilde R_b$. Therefore, we are able to cancel it by choosing $y=1$. We proceed with
\beq
\omega_1=a, \quad \omega_2=c, \quad \omega_3=d, \qquad\qquad 
R_1=\tilde R_a,\quad R_2=\tilde R_c, \quad R_3=\tilde R_d.\quad    
\eeq  
The corresponding potential is shown in Fig. \ref{3S1BP} (section \ref{simplest}).

Finally, we consider a $(4,1)[1]^+$ type S-matrix composed of 5 factors
\beq
S(k)=\sigma_a(k)\sigma_b(k)\sigma_c(k)\sigma_d(k)\sigma_e(k),
\eeq
with one of its poles being negative \cite{X}:
\beq
a=-0.45146,\quad b=0.23154,\quad c=0.43654, \quad d=1.6818, \quad e=2.3106. 
\eeq 
Once again, the bound state momentum is $\kappa_o=b$. Since the contour is closed in upper half plane, we observe that the negative pole does not contribute to the integral (\ref{Fs2}). Therefore, we obtain
\beq
F(r)=(y-1)\tilde R_b{\rm e}^{-br}-\tilde R_c{\rm e}^{-cr}-\tilde R_d{\rm e}^{-dr}-\tilde R_e{\rm e}^{-er},
\eeq  
where 
\begin{eqnarray}
\tilde R_b&=& 2b\frac{(b+a)(b+c)(b+d)(b+e)}{(b-a)(b-c)(b-d)(b-e)},\quad \tilde R_c= 2c\frac{(c+a)(c+b)(c+d)(c+e)}{(c-a)(c-b)(c-d)(c-e)},\\ \qquad \quad
\tilde R_d&=& 2d\frac{(d+a)(d+b)(d+c)(d+e)}{(d-a)(d-b)(d-c)(d-e)}, \quad \tilde R_e= 2e\frac{(e+a)(e+b)(e+c)(e+d)}{(e-a)(e-b)(e-c)(e-d)}.  \qquad \quad
\end{eqnarray} 
We again focus on the $y=1$ case and write 
\begin{equation}
%\begin{align}
\omega_1=c, \quad \omega_2=d, \quad \omega_3=e,\qquad\qquad
R_1=\tilde R_c, \quad R_2=\tilde R_d, \quad R_3=\tilde R_e.
%\end{align}
\end{equation}
The corresponding potential is shown in Fig. \ref{3S1X} (section \ref{simplest}).


==> sing.tex <==
Quantum inverse scattering is the problem of finding the potential from 
scattering data. Its complete solution is known in the one-dimensional
case \cite{QIS1a,QIS1b,QIS1c} both for the entire line and the half line
cases. Here we will consider the latter case because the same mathematical
problem emerges for three-dimensional spherically symmetric potentials after
partial wave expansion. The details of the inversion procedure depend on
the class of potentials. The simplest case is that of regular potentials
\cite{QIS2}. We will proceed along the lines presented in \cite{QIS2},
generalized to the case of potentials with a singular core at the origin.

The radial part of the Schr\"odinger equation for the wave function
\beq
\psi(r)=\frac{u(r)}{r},\qquad\quad r>0
\eeq
is of the form
\beq
-\frac{\hbar^2}{2m}u^{\prime\prime}(r)+\frac{\hbar^2}{2m}\,\frac{\ell(\ell+1)}
{r^2}u(r)+V(r)u(r)=Eu(r),
\eeq
where $V(r)$ is the interaction potential, $m$ is the reduced mass,
$\ell$ is the angular momentum quantum number and
$E$ is the energy of the system. After rescaling the variables as
\beq
V(r)=\frac{\hbar^2}{2m}w(r),\qquad\quad E=\frac{\hbar^2 k^2}{2m}, 
\eeq
the Schr\"odinger equation becomes
\beq
-u^{\prime\prime}(r)+q(r)u(r)=k^2u(r)
\label{diff}
\eeq
with
\beq
q(r)=w(r)+\frac{\ell(\ell+1)}{r^2}.
\eeq
For simplicity here we will restrict our attention to the s-wave problem
$\ell=0$, where the centrifugal term is absent from the Schr\"odinger equation.
The Schr\"odinger differential operator (defined by the left hand side of
(\ref{diff})) is made self-adjoint by the natural boundary condition $u(0)=0$.

We will assume that the everywhere smooth potential $q(r)$ is strongly
repulsive at the origin:
\beq
q(r)\sim\frac{p(p-1)}{r^2},\qquad\quad r\to0,
\eeq
with $p>1$. (Results for regular potentials are recovered in the limit
$p\to1$.) We also assume that $q(r)$ vanishes exponentially for $r\to\infty$.

\subsection{Direct scattering}

For a given $k$, we define three special solutions of the differential 
equation (\ref{diff}). The physical solution $\varphi(r,k)$ is defined by
its regular behaviour near the origin,
\beq
\varphi(r,k)=r^p[1+{\rm O}(r)],\qquad\quad r\to0.
\eeq
The singular solution $\tilde\varphi(r,k)$ is defined by the requirement
\beq
\tilde\varphi(r,k)=r^{1-p}[1+{\rm O}(r)],\qquad\quad r\to0
\eeq
and the absence of the $r^p$ term in its small $r$ expansion.
The Jost solution is defined by its large $r$ asymptotics
\beq
f(r,k)={\rm e}^{ikr}[1+{\rm O}(1/r)],\qquad\quad r\to\infty.
\eeq

Since (\ref{diff}) is of second order, any of the above three solutions
can be expressed as a linear combination of the other two.
Let us write the Jost solution as
\beq
f(r,k)=\tilde f(k)\varphi(r,k)+f(k)\tilde\varphi(r,k)
\label{lin1}
\eeq
with some coefficients $\tilde f(k)$, $f(k)$. $f(k)$ is called the Jost
function and plays an important role in scattering theory\footnote{For the
case of regular potentials $\varphi(0,k)=0$, $\tilde\varphi(0,k)=1$
and $f(k)$ is simply given by $f(0,k)$.}. It is easy to see that
an alternative definition of $f(k)$ is given by the linear combination
coefficients in
\beq
\varphi(r,k)=\frac{2p-1}{2ik}\left\{f(-k)f(r,k)-f(k)f(r,-k)\right\}.
\label{lin2}
\eeq
For real $k$
\beq
f^*(r,k)=f(r,-k)\qquad\qquad{\rm and}\qquad\qquad
f^*(k)=f(-k)
\eeq
and if we introduce the modulus and phase of $f(k)$ by writing
\beq
f(k)=\vert f(k)\vert{\rm e}^{-i\delta(k)}
\eeq
we see that
\beq
\vert f(k)\vert=\vert f(-k)\vert\qquad{\rm and}\qquad \delta(-k)=
-\delta(k)\quad{\rm mod\ }2\pi.
\eeq

The Jost solutions and functions are first defined for real $k$, but they
can be analytically continued and become analytic in the entire upper $k$
half-plane. If for large $r$ $q(r)$ decays fast enough, they become meromorphic
functions in the entire $k$ plane (with pole singularities in the lower
half-plane). The symmetry relations become
\beq
f^*(r,k)=f(r,-k^*)\qquad\qquad{\rm and}\qquad\qquad
f^*(k)=f(-k^*).
\eeq

In addition to the scattering solutions with real momentum $k$, the
Schr\"odinger equation (\ref{diff}) can have normalizable bound state solutions
with imaginary $k=i\kappa_j$, $j=1,...,J$ (negative energy). There is a bound
state solution with (rescaled) energy $-\kappa_j^2$ whenever
\beq
f(i\kappa_j)=0.
\eeq
In this case
\beq
\varphi_j(r)=\varphi(r,i\kappa_j)\qquad
{\rm and}\qquad
f_j(r)=f(r,i\kappa_j)
\eeq
are normalizable and are related by
\beq
f_j(r)=\tilde f(i\kappa_j)\varphi_j(r).
\eeq
All zeroes of $f(k)$ in the upper half-plane correspond to bound states and
$f(k)\not=0$ for real $k\not=0$. $f(0)$ may be vanishing, but this does not
correspond to any bound state.
The norming constants
\beq
\frac{1}{c_j}=\int_0^\infty{\rm d}r\varphi_j^2(r),\qquad
\frac{1}{s_j}=\int_0^\infty{\rm d}rf_j^2(r),\qquad
\eeq
are important quantities in inverse scattering theory. If we introduce the
normalized bound state wave function $\psi_j$, we can write
\beq
\psi_j(r)=\sqrt{c_j}\varphi_j(r)={\rm sgn}[\tilde f(i\kappa_j)]\sqrt{s_j}f_j(r).
\eeq
The norming constants $s_j$ can be expressed as \cite{QIS2}
\beq
s_j=-\frac{2i\kappa_j}{(2p-1)f^\prime(i\kappa_j)\tilde f(i\kappa_j)}.
\eeq
From this it follows that
\beq
{\rm sgn}[\tilde f(i\kappa_j)]={\rm sgn}[if^\prime(i\kappa_j)]
\eeq
and the asymptotic behaviour of the normalized wave function is given by
\beq
\psi_j(r)=A_jf_j(r)\sim A_j{\rm e}^{-\kappa_j r},\qquad r\to\infty,
\eeq
where
\beq
A_j={\rm sgn}[if^\prime(i\kappa_j)]\sqrt{s_j}.
\eeq

We define the \lq\lq S-matrix'' $S(k)$ by
\beq
S(k)=\frac{f(-k)}{f(k)}={\rm e}^{2i\delta(k)},
\eeq
where $\delta(k)$ is the phase shift. $S(k)$ enjoys the symmetry properties
\beq
S(-k)=\frac{1}{S(k)}=S^*(k).
\label{syms}
\eeq
If $f(0)\not=0$, $S(0)=1$, but if $f(0)=0$, $S(0)$ may be also $-1$.
We introduce the variables
\beq
\mu=S(0),\qquad\qquad \Delta=\frac{1-\mu}{2}.
\eeq
In the meromorphic case $S(k)$ is also meromorphic in the whole complex plane.
In some cases (not always) $S(k)$ has pole at $k=i\kappa_j$.
If this is the case, it is often (but not always) true that
the norming constant $s_j$ is related to the residue of the pole:
\beq
s_j=\hat s_j,\qquad\quad{\rm where}\qquad \hat s_j=
i{\rm Res}[S(k)]{\big|}_{k=i\kappa_j}.
\label{RQFT}
\eeq
It is known that in relativistic quantum field theory there is a relation
between bound states and S-matrix poles. If our Schr\"odinger equation
is an effective quantum mechanical representation of a system originally
described by quantum field theory, the S-matrix is always singular at the
position of the bound states and also (\ref{RQFT}) is satisfied. 

The large $k$ behaviour of the Jost function in the upper half-plane is
\beq
f(k)\approx\frac{\Gamma(2p-1)}{\Gamma(p)}(-2ik)^{1-p}[1+{\rm O}(1/k)].
\eeq
From this it follows that for large positive $k$
\beq
\delta(k)=\frac{\pi}{2}(1-p)+{\rm O}(1/k),\qquad\quad\delta(\infty)=
\frac{\pi}{2}(1-p).
\eeq
Since (mod $2\pi$) $\delta(-\infty)=-\delta(\infty)$, $S(\infty)$
and $S(-\infty)$ are not the same in general, except for integer $p$,
in which case
\beq
S(\infty)=S(-\infty)=(-1)^{p-1}.
\eeq

From (\ref{lin2}) we see that  for large $r$ asymptotically
\beq
\varphi(r,k)\approx -\frac{2p-1}{2ik}f(k)\left\{{\rm e}^{-ikr}-S(k){\rm e}^{ikr}
\right\}=\frac{2p-1}{k}\vert f(k)\vert\sin[kr+\delta(k)].
\eeq
Thus $\delta(k)$ can indeed be identified as the phase shift.

Finally we recall Levinson's theorem, which in our case takes the form \cite{Swan}
\beq
\delta(\infty)-\delta(0)=\frac{1}{2}\int_{-\infty}^\infty{\rm d}k\,
\delta^\prime(k)=-\frac{\pi}{2}[2J+\Delta+p-1].
\label{Levi}
\eeq



\subsection{Inverse scattering}

We will use Marchenko's method to find the potential from given scattering data.
The latter is the set
\beq
{\cal S}=\left\{S(k);\{\kappa_j,s_j\}_{j=1}^J\right\}.
\eeq
We see that any given S-matrix must be supplemented by $2J$ additional
parameters, the positions $\kappa_j$ of the bound states and the corresponding
norming constants $s_j$. ${\cal S}$ is only constrained by Levinson's theorem
(\ref{Levi}).

Inverse scattering now proceeds in three steps. The first step is to
calculate the function
\beq
F(r)=F_b(r)+F_s(r),
\eeq
where
\beq
F_b(r)=\sum_{j=1}^J s_j\,{\rm e}^{-\kappa_j r}
\eeq
and
\beq
F_s(r)=\frac{1}{2\pi i r}\int_{-\infty}^\infty{\rm d}k\,{\rm e}^{ikr} S^\prime(k).
\eeq
If $p$ is integer, after partial integration we get
\beq
F_s(r)=\frac{1}{2\pi}\int_{-\infty}^\infty{\rm d}k\,{\rm e}^{ikr}
[S(\infty)-S(k)].
\label{Fs2}
\eeq
For $p=1$ the standard formula \cite{QIS2} is reproduced.

The second step is to find the kernel $A(r,u)$ by solving the
Marchenko equation 
\beq
F(r+u)+A(r,u)+\int_r^\infty{\rm d}t\,A(r,t)\,F(t+u)=0,\qquad\quad u>r>0.
\label{Marchenko}
\eeq

The third and final step is to use the formula
\beq
q(r)=-2\frac{{\rm d}}{{\rm d}r}A(r,r)
\label{third}
\eeq
to determine $q(r)$.

The transformation kernel $A(r,u)$ can be used to define the linear operator
$\hat{\cal A}$ which maps the solutions of the free problem onto those
of the interacting problem with potential $q(r)$. The action of $\hat{\cal A}$
is defined by
\beq
\big(\hat{\cal A}{\cal F}\big)(r)={\cal F}(r)+\int_r^\infty{\rm d}u
A(r,u){\cal F}(u)
\eeq
and the mapping is
\beq
f_k=\hat{\cal A}E_k,\qquad\qquad f_k(r)=f(r,k),\qquad E_k(r)={\rm e}^{ikr}.
\eeq
For $k=i\kappa_j$ we find
\beq
f_j=\hat{\cal A}\,\varepsilon_j,\qquad\qquad \varepsilon_j(r)={\rm e}^{-\kappa_j r}.
\eeq

